CheXNet: Radiologist-Level Pneumonia Detection on Chest X-Rays with Deep Learning

We develop an algorithm that can detect pneumonia from chest X-rays at a level exceeding practicing radiologists. Our algorithm, CheXNet, is a 121-layer convolutional neural network trained on ChestX-ray14, currently the largest publicly available chest X-ray dataset, containing over 100,000 frontal-view X-ray images with 14 diseases. Four practicing academic radiologists annotate a test set, on which we compare the performance of CheXNet to that of radiologists. We find that CheXNet exceeds average radiologist performance on the F1 metric. We extend CheXNet to detect all 14 diseases in ChestX-ray14 and achieve state of the art results on all 14 diseases.

==> discussion.tex <==
\section{Discussion}

% The evaluation environment of the radiologists in this study was limited for four important reasons: (1) the reporting task required the radiologists to choose from a predefined list of abnormalities, which is a very different practice from the freestyle reporting that radiologists are accustomed to,
% % the reporting task using a list of possible abnormalities is very different from the ``freestyle'' reporting that radiologists are accustomed to in most environments, 
% (2) the radiologists were not permitted to use prior or comparison examinations, which has been shown to decrease radiologist performance \cite{Berbaum1985} (for example, interstitial pulmonary fibrosis would be a chronic finding identified on many prior chest radiographs over time while interstitial edema would be acute and varying over time),
% % , thus the task of honing in on the relevant pathology in the context of only one image likely limited radiologist accuracy , 
% (3) the radiologists were not permitted to use patient history, which has been shown to decrease radiologist diagnostic performance in interpreting chest radiographs (for example, given a pulmonary abnormality with a history of fever and cough, pneumonia would be appropriate rather than less specific terms such as infiltrate or consolidation) \cite{Potchen1979}, (4) only frontal radiographs were presented to the radiologists during diagnosis, and it has been shown that up to 15 percent of accurate diagnoses require the lateral view \cite{raoof2012interpretation}. It is also important to mention the ambiguity around terms like infiltrate which are non-specific with regard to the imaging appearance, particularly if pneumonia and consolidation are included as alternate options. In particular, infiltrate remains a controversial term for pulmonary disease in radiography and many practices discourage its use \cite{Patterson2005}.

% Pneumonia accounts for a significant patient morbidity and mortality, especially the population who needed mechanical ventilation or vasopressor support \cite{gonccalves2013community}. Thus, early diagnosis and treatment of pneumonia is critical to prevent complications, including loss of life \cite{aydogdu2010mortality}. Chest radiographs are the most common radiological investigations in health care and are critical for screening, diagnosis, and management of a variety of diseases including pneumonia \cite{raoof2012interpretation}.

% The interpretation of chest radiographs is a complex task that is prone to diagnostic error; for example a study evaluating the accuracy of a pneumonia diagnosis using chest radiographs found that the diagnosis missed 28 percent of cases, and was even less accurate when the patient was older and under nursing home care \cite{miyashita2015detection}. In another study, an independent, blinded comparison of chest radiography with high-resolution computed tomography confirmation, chest radiography interpretations missed 31 percent of pneumonia cases \cite{syrjala1998high} Thus, the motivation for a deep learning model to aid in the interpretation task would aim to overcome the intrinsic limitations of human perception and bias to reduce errors in interpretation. More broadly, we believe that a deep learning model for this purpose could improve health care delivery across a wide range of settings; in the case of chest radiography the treating physician often initially reviews and interprets the examinations and makes clinical decisions before the exam can be reviewed in the radiology workflow. A deep learning model could aid in the interpretation of chest radiography in the clinical setting prior to radiologist review, potentially decreasing the discordance rate and improving patient care in the outpatient or emergency clinical setting.  Future studies are needed to evaluate whether deep learning models, such as the one presented here, can significantly improve diagnostic accuracy in the clinical setting.

% %One immediately translatable application for the model described in this paper could be for radiologist worklist prioritization.  In this scenario, the x-rays that the model automatically identifies as abnormal can be moved ahead in the workflow prioritization during the image interpretation task, leading to the sickest patients receiving diagnoses from radiologists in a more timely manner; this could mean more rapid results can be conveyed to the ordering provider (and patient) which would improve disposition in other areas of the healthcare system (i.e. discharged from the ED more quickly).  Another powerful potential application of this model could be as an "intelligent" computer aided detection (CAD) in which the model would automatically create a color coded “map” that would mark the portion of the image that the model recognized as abnormal drawing the attention of the clinician. The model could be continually trained with feedback from the radiologist (as oppsoed to the static models in existing CAD) such that the model could "learn" from false positives/false negatives via iterative real-time feedback.  The resulting "intelligent" CAD could lead to more efficient interpretation of the imaging examination, reduce errors, and helping to standardize quality.   

% Finally, the World Health Organization estimates that two thirds of the world’s population lacks access to radiology diagnostics \cite{mollura2010white}. Yet, radiology is critical for the diagnosis and treatment of many diseases; in many instances even when imaging equipment is available there are often no physicians with the expertise to perform interpretation, leading to misdiagnosis, delayed treatment, spread of communicable disease, and ultimately increased mortality from treatable diseases \cite{kesselman20162015}. We believe that our work and other similar efforts could help lead to a cost-effective approach to aid efforts in resource poor areas of the world that have imaging equipment but limited or no access to radiologists for the detection of diseases such as pneumonia (including TB), as well as other diseases such as cancer, trauma, HIV, and more.




